Electromagnetic Sensor and Actuator Attacks on Power Converters for Electric Vehicles

Alleviating range anxiety for electric vehicles (i.e., whether such vehicles can be relied upon to travel long distances in a timely manner) is critical for sustainable transportation. Extremely fast charging (XFC), whereby electric vehicles (EV) can be quickly recharged in the time frame it takes to refuel an internal combustion engine, has been proposed to alleviate this concern. A critical component of these chargers is the efficient and proper operation of power converters that convert AC to DC power and otherwise regulate power delivery to vehicles. These converters rely on the integrity of sensor and actuation signals. In this work the operation of state-of-the art XFC converters is assessed in adversarial conditions, specifically against Intentional Electromagnetic Interference Attacks (IEMI). The targeted system is analyzed with the goal of determining possible weak points for IEMI, viz. voltage and current sensor outputs and gate control signals. This work demonstrates that, with relatively low power levels, an adversary is able to manipulate the voltage and current sensor outputs necessary to ensure the proper operation of the converters. Furthermore, in the first attack of its kind, it is shown that the gate signal that controls the converter switches can be manipulated, to catastrophic effect; i.e., it is possible for an attacker to control the switching state of individual transistors to cause irreparable damage to the converter and associated systems. Finally, a discussion of countermeasures for hardware designers to mitigate IEMI-based attacks is provided.

==> Figure/AttackEM.tex <==
\begin{tikzpicture}[cross/.style={path picture={\draw[black] (path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east);}}]

%z,x
\draw[->] (0,0) -- (0,1.5);
\node[anchor=south] at (0,1.5) {$z$};

\draw[->] (0,0) -- (2.75,0);
\node[anchor=west] at (2.75,0) {$x$};

%current
\draw (-0.15,-1.25) -- node[left] {$i(t)$} (-0.15,1.25);
\draw[->,red,thick] (0,-0.9) -- (0,0.9);
\draw (0.15,-1.25) -- (0.15,1.25);

%surface
\draw[dashed] (1.25,0.05) -- (1.25,1) -- (2.25,1) -- (2.25,0.05) --
(1.25,0.05);
\node[anchor=south] at (2.25,1) {$\mathcal{S}$};

%load
\filldraw[fill=white, draw=black] (2.15,0.25) rectangle
(2.35,0.75);
\node[anchor=west] at (2.35,0.5) {$v(t)$};

%field
\node [draw,circle,cross,minimum width=0.25 cm,label={$\mathbf{H}$}](B) at (0.75,1){}; 

%dimensions
\draw[decorate,decoration={brace,mirror,raise=2pt},black] (0.15,0) --
node[below,black,yshift=-2pt] {$d$} (1.25,0);
\draw[decorate,decoration={brace,mirror,raise=2pt},black] (1.25,0) --
node[below,black,yshift=-2pt] {$a$} (2.25,0);
\draw[decorate,decoration={brace,raise=2pt},black] (1.25,0) --
node[left,black,xshift=-2pt] {$b$} (1.25,1);


\end{tikzpicture}
